Search for high-mass resonances decaying to dilepton final states in pp collisions at a center-of-mass energy of 7 TeV with the ATLAS detector

The ATLAS detector at the Large Hadron Collider is used to search for high-mass resonances decaying to an electron-positron pair or a muon-antimuon pair. The search is sensitive to heavy neutral Z' gauge bosons, Randall-Sundrum gravitons, Z* bosons, techni-mesons, Kaluza-Klein Z/gamma bosons, and bosons predicted by Torsion models. Results are presented based on an analysis of pp collisions at a center-of-mass energy of 7 TeV corresponding to an integrated luminosity of 4.9/fb in the dielectron channel and 5.0/fb in the dimuon channel. A Z' boson with Standard Model-like couplings is excluded at 95 percent confidence level for masses below 2.22 TeV. A Randall-Sundrum graviton with coupling k/Mbar = 0.1 is excluded at 95 percent confidence level for masses below 2.16 TeV. Limits on the other models are also presented, including Technicolor and Minimal Z' Models.

==> strategy.tex <==
 strategy.tex


The dilepton invariant mass (\mll) spectrum measured in the data must be compared to the SM prediction.
The comparison is then performed in the search region $0.13<\mll <3.0$~TeV by means of templates~\cite{Aad:2011xp, CDF:Zpmumu2fb}.
The templates provide the expected yield of events ($\bar{n}$) in each \mll\ bin. 
$\bar{n}$ is given by $\bar{n} = n_X(\lambda , {\pmb\nu}) + n_{\dy} ({\pmb\nu}) + \nobg ({\pmb\nu})$ when neglecting interference,
and $\bar{n} = n_{X+\dy}(\lambda , {\pmb\nu}) + \nobg ({\pmb\nu})$ when including  the effects of interference. 
In the definition of $\bar{n}$, $\lambda$ represents the parameter of interest of the model, 
$n_{X}$, $n_{\dy}$ and \nobg\ represent the number of 
signal events for model $X$,
\dy\ (Drell-Yan) and other backgrounds, respectively.
${\pmb\nu}$ is the set of Gaussian-distributed nuisance parameters incorporating the systematic uncertainties.

Signal templates, that is $n_X(\lambda , {\pmb\nu})$ as a function of \mll , provide the expected line-shape of the dilepton resonances.
%

Most of the dilepton resonances searched for in this analysis are narrow compared to the detector resolution.
The effect of width variations on the resonance line-shape is neglected for the \esix\ analysis.
On the other hand, the dependence of the width on the coupling strength  
is taken into account in 
the MWT, Torsion and \gstar\ analyses by using several templates for a given pole mass 
in which various values of the couplings were selected. 
%
Signal templates include the acceptance times efficiency of the signal, at a given pole mass $M_X$, over the full search region.
The product \acc\ is different for each model due to different angular distributions, boosts, and line-shapes.

%% statistical treatment 
The most likely number of signal events, and the corresponding confidence intervals, 
 are determined from a likelihood function  defined as the product of the Poisson probabilities over all mass bins in the search region.
% 
For \zkk\ and the Minimal \zp\ Models, the most likely value of the coupling strength is determined instead of the number of signal events.
For \zkk, 
this is mandatory because of the strong interference which prevents the signal from being defined independently from the \dy\ contribution.
The Minimal \zp\ Models have only two parameters, a coupling and a mixing angle, and the aim is to set a limit on the coupling.

The same Bayesian approach~\cite{bayesianMethod} is used in all cases,
with a flat prior on the signal cross section times branching fraction (\xbr) when neglecting interference 
or on the coupling strength to the second or fourth power when including the effects of interference.
The nuisance parameters are integrated out.


